Timed context-free temporal logics (extended version)

The paper is focused on temporal logics for the description of the behaviour of real-time pushdown reactive systems. The paper is motivated to bridge tractable logics specialized for expressing separately dense-time real-time properties and context-free properties by ensuring decidability and tractability in the combined setting. To this end we introduce two real-time linear temporal logics for specifying quantitative timing context-free requirements in a pointwise semantics setting: Event-Clock Nested Temporal Logic (ECNTL) and Nested Metric Temporal Logic (NMTL). The logic ECNTL is an extension of both the logic CARET (a context-free extension of standard LTL) and Event-Clock Temporal Logic (a tractable real-time logical framework related to the class of Event-Clock automata). We prove that satisfiability of ECNTL and visibly model-checking of Visibly Pushdown Timed Automata VPTA against ECNTL are decidable and EXPTIME-complete. The other proposed logic NMTL is a context-free extension of standard Metric Temporal Logic (MTL). It is well known that satisfiability of future MTL is undecidable when interpreted over infinite timed words but decidable over finite timed words. On the other hand, we show that by augmenting future MTL with future context-free temporal operators, the satisfiability problem turns out to be undecidable also for finite timed words. On the positive side, we devise a meaningful and decidable fragment of the logic NMTL which is expressively equivalent to ECNTL and for which satisfiability and visibly model-checking of VPTA are EXPTIME-complete.

==> DecisionProcedures.tex <==

\section{Decision procedures for B\"{u}chi \ECNA}\label{sec:DecisionProcedures}

In this section, we investigate the following decision problems:
%
\begin{itemize}
  \item Emptiness,  universality, and language inclusion for B\"{u}chi \ECNA.
  \item \emph{Visibly model-checking problem:} given a \emph{visibly pushdown timed system $\mathcal{S}$} over $\Sigma_\Prop$ (that is a B\"{u}chi \VPTA\ where all the states are accepting)
  and a B\"{u}chi \ECNA\ $\Au$ over  $\Sigma_\Prop$,   does $\TLang(\mathcal{S})\subseteq \TLang(\Au)$ hold?
\end{itemize}
%
We establish that the above problems are decidable and \EXPTIME-complete. The key intermediate result is an exponential-time translation
of B\"{u}chi \ECNA\ $\Au$ into language-equivalent generalized B\"{u}chi \VPTA. More precisely, we show that event-clocks in nested \VPTA\ can be removed with a single exponential blow-up.


\begin{theorem}[Removal of event-clocks from nested \VPTA]\label{theorem:FromECNAtoVPTA}
Given a generalized B\"{u}chi \emph{nested} \VPTA\ $\Au$, one can construct in singly exponential time a generalized B\"{u}chi   \VPTA\ $\Au'$ which do not use event-clocks such that
$\TLang(\Au')=\TLang(\Au)$ and $K_{\Au'}=K_{\Au}$. Moreover, $\Au'$ has $n_s\cdot 2^{O(n_e)}$ states and $n_c + O(n_e)$ clocks, where $n_s$ is the number of $\Au$-states, $n_c$ is the number
of $\Au$-clocks, and $n_e$ is the number of \emph{event-clock} atomic constraints used by $\Au$.
\end{theorem}

In the following, we illustrate the proof of Theorem~\ref{theorem:FromECNAtoVPTA}. The translation in  Theorem~\ref{theorem:FromECNAtoVPTA} consists of a sequence of steps preserving language equivalence,
where at each step, we remove one event-clock and replace it with a set of fresh normal clocks. The removal of global predictor and recorder event-clocks is done as illustrated in \cite{}.
Here, we describe how to remove an \emph{abstract predictor} event-clock $y^{\abs}_p$ where $p\in \Prop$ (the treatment of abstract recorder event-clocks is similar, and is described in Appendix~\ref{APP:RemovalAbstractRecorder}).
Fix a generalized B\"{u}chi nested \VPTA\ $\Au=\tpl{\Sigma_\Prop, Q,Q_{0},C'=C\cup C_n,\Gamma\cup\{\top\},\Delta,\mathcal{F}}$ such that $y^{\abs}_p \in C$.
By exploiting nondeterminism, we can assume that for each transition $\delta$ of $\Au$, there is exactly one atomic constraint $y^{\abs}_p\in I$ involving $y^{\abs}_p$ occurring as conjunct in the clock constraint
of $\delta$.  If $I\neq \{\NULL\}$, then   $y^{\abs}_p\in I$ is equivalent to a constraint of the form $y_p^{\abs}\succ \ell \wedge y_p^{\abs} \prec u$, where $\succ \in \{>,\geq\}$, $\prec\in \{<,\leq\}$,
$\ell \in \Nat$, and $u\in \Nat\cup\{\infty\}$. We call $y_p^{\abs}\succ \ell$ a lower-bound constraint and $y_p^{\abs} \prec u$ an upper bound constraint. Note that if $u=\infty$ , the constraint $y_p^{\abs} \prec u$
is always fulfilled, but we include it for allowing a uniform notation.
We construct a generalized B\"{u}chi nested \VPTA\ $\Au_{y^{\abs}_p }$ equivalent to $\Au$ whose set of event-clocks is  $C\setminus \{y^{\abs}_p\}$, and whose set of normal clocks is
$C\cup C_\new$, where $C_\new$ consists of the  fresh normal clocks $z_{\succ \ell}$ (resp., $z_{\prec u}$), for each lower bound constraint  $y_p^{\abs}\succ \ell$  (resp., upper bound constraint $y_p^{\abs} \prec u$)
of $\Au$ involving $y_p^{\abs}$.

We first explain the basic ideas of the translation. Let us consider a lower-bound constraint $y_p^{\abs} \succ \ell$. Assume that a prediction $y_p^{\abs} \succ \ell$ is done by the automaton $\Au$
at position $i$ of the input word for the first time. Then, the simulating automaton $\Au_{y^{\abs}_p}$ exploits the normal clock $z_{\succ \ell}$ for checking that the prediction
holds by resetting it at position $i$. Moreover, if $i$ is not a call (resp., $i$ is a call), $\Au_{y^{\abs}_p}$ carries the obligation $\succ$$\ell$ in its control state (resp., pushes the obligation $\succ$$\ell$ onto the stack)
in order to check that  along the maximal abstract path (\MAP, for short) $\nu$ visiting position $i$, when the next $p$ occurs at a position $j_{\textit{check}}$,  the constraint  $z_{\succ \ell}\succ \ell$ holds.
The crucial observation is that:
\begin{compactitem}
  \item if a new prediction $y_p^{\abs} \succ \ell$ is done by the automaton $\Au$ along a position $j>i$ of   $\nu$ strictly preceding  $j_{\textit{check}}$, $\Au_{y^{\abs}_p}$ replaces the old obligation with the new one by resetting
  the clock $z_{\succ \ell}$ at the current position $j$. This is safe since the fulfillment of the lower-bound prediction $y_p^{\abs} \succ \ell$ at position $j$  implies the fulfillment of the
  prediction  $y_p^{\abs} \succ \ell$ at the previous position $i$ along $\nu$.
  \item If a call position $i_c\geq i$ occurs along $\nu$ before $j_{\textit{check}}$, we know that the next position of $i_c$  along $\nu$ is the matching return $i_r$ of $i_c$, and all the \MAP\ visiting positions
  $h\in [i_c+1,i_r-1]$ are finite and terminate at positions $k<i_r$. Thus, the fulfillment of a prediction $y_p^{\abs} \succ \ell$ done along such \MAP\ always implies the fulfillment of the prediction done at position $i$.
  Therefore, for such predictions, the clock $z_{\succ \ell}$ can be safely reset.
\end{compactitem}\vspace{0.2cm}

\noindent Thus, previous obligations on a lower-bound constraint $y_p^{\abs} \succ \ell$ are always discarded in favour of new ones. At each non-return position $i$, $\Au_{y^{\abs}_p}$ keeps tracks in its control state
of the lower-bound obligations for the current \MAP\ $\nu$ (i.e., the \MAP\ visiting the current position $i$). Whenever  a call $i_c$ occurs, the lower-bound obligations are pushed on the stack in order to be recovered at the matching return $i_r$ of $i_c$. Moreover, if $i_c+1$ is not a return (i.e., $i_r\neq i_c+1$), then $\Au_{y^{\abs}_p}$ moves to a control state where the set of lower-bound obligations is empty (consistently with the fact that $i_c+1$ is the initial position of the \MAP\ visiting $i_c+1$).

The situation for a upper-bound constraint $y_p^{\abs}  \prec u$ is dual. Whenever a prediction $y_p^{\abs}  \prec u$ is done by $\Au$ at a position $i$, and the simulating automaton $\Au_{y^{\abs}_p}$ has no obligation  concerning the constraint $y_p^{\abs}  \prec u$, $\Au_{y^{\abs}_p}$ resets the normal clock $z_{\prec u}$ and carries the fresh obligation ($\first$,$\prec$$u$) in its control state (resp., pushes the obligation ($\first$,$\prec$$u$) onto the stack) if $i$ is not a call (resp., $i$ is a call). When, along the \MAP\ $\nu$ visiting position $i$, the next $p$ occurs at a position $j_{\textit{check}}$,   the constraint  $z_{\prec u}\prec u$ is checked, and the obligation ($\first$,$\prec$$u$) is removed or confirmed (in the last case, resetting the clock $z_{\prec u}$), depending on whether the prediction $y_p^{\abs}  \prec u$ is asserted at position  $j_{\textit{check}}$ or not. The crucial observation is:
\begin{compactitem}
  \item if a new prediction $y_p^{\abs} \prec u$ is done by the automaton $\Au$ along a position $j>i$ of   $\nu$ strictly preceding  $j_{\textit{check}}$, $\Au_{y^{\abs}_p}$ simply ignores the new prediction (the clock $z_{\prec u}$  is not reset at position $j$) since it is subsumed by the current one. Indeed,  the fulfillment of the upper-bound prediction $y_p^{\abs} \prec u$ at the previous position $i$  implies the fulfillment of the
  prediction  $y_p^{\abs} \prec u$ at the current position $j>i$ along $\nu$.
  \item If a call position $i_c\geq i$ occurs along $\nu$ before $j_{\textit{check}}$, then all the predictions $y_p^{\abs}  \prec u$ done along the \MAP\ associated to the positions
  $h\in [i_c+1,i_r-1]$, where $i_r\leq j_{\textit{check}}$ is the matching-return of $i_c$, can be safely ignored (i.e., the clock $z_{\prec u}$ is not reset along these positions) since they are subsumed by the prediction done at position $i$.
\end{compactitem}\vspace{0.2cm}


\noindent Thus, new obligations on an upper-bound constraint $y_p^{\abs} \prec u$ are always ignored (i.e, the clock $z_{\prec u}$ is not reset). Whenever a
call $i_c$ occurs, the updated set $O$ of  upper-bound and lower-bounds obligations   are pushed onto the stack  in order to be recovered at the matching return $i_r$ of $i_c$.
Moreover, if $i_c+1$ is not a return (i.e., $i_r\neq i_c+1$), then $\Au_{y^{\abs}_p}$ moves to a control state where, while the set of lower-bound obligations is empty, the set $U$ of upper-bound  obligations is
obtained from $O$ by replacing each upper-bound obligation ($f$,$\prec$$u$), where $f\in \{\live,\first\}$ with the live obligation ($\live$,$\prec$$u$). A live obligation ($\live$,$\prec$$u$) asserted at the initial position
$i_c+1$ of the \MAP\  $\nu$ visiting $i_c+1$ (note that $\nu$ terminates at position $i_r-1$) is used by $\Au_{y^{\abs}_p}$ to remember that the clock $z_{\prec u}$ cannot be reset along $\nu$. Intuitively, live upper-bound obligations are propagated from the caller \MAP\ to the called \MAP. Note that fresh upper-bound obligations $(\first,\prec$$ u)$ always refer to predictions done along the current \MAP\, and differently form the live upper-bound obligations, can be removed, when along the current \MAP, the next $p$ occurs.

There are other technical issues to be handled. At each position $i$, the automaton $\Au_{y^{\abs}_p}$ guesses whether $i$ is the last position of the current \MAP\ (i.e., the \MAP\ visiting $i$) or not.
For this, it keep tracks in its control state of the guessed type (call, return, or internal symbol) of the next input symbol. In particular, when $i$ is a call,
$\Au_{y^{\abs}_p}$ guesses whether the call $i$ has a matched-return or not. In the second case, $\Au_{y^{\abs}_p}$ pushes onto the stack a special symbol, say $\bad$, and the guess is correct iff
the symbol is never popped from the stack. For the first case, the automaton exploits a special proposition $p_{\infty}$ whose Boolean value is carried in the control state:
$p_{\infty}$ \emph{does not hold} at a position $i$ of the input iff the \MAP\ visiting $i$ starts at a position $j>0$ such that $j-1$ is a matched call (i.e., position $i$ has a caller whose
matching return exists). A B\"{u}chi component of $\Au_{y^{\abs}_p}$ consists of the states where the Boolean value of $p_{\infty}$ is $\true$.
Finally, we have to ensure that the lower-bound obligations and fresh upper-bound obligations at the current position  $i$ are eventually checked, i.e., the current \MAP\ eventually visits a position
where $p$ holds. For this, the automaton exploits the \CARET\ \cite{} formula $\Eventually^{\abs}p$ whose Boolean value is carried in the control state:
$\Eventually^{\abs}p$ holds at a position $i$ if the \MAP\ visiting $i$ also visits a position $j\geq i$, where $p$ holds.  A B\"{u}chi component of $\Au_{y^{\abs}_p}$ ensures  the fulfillment of the liveness requirement
$p$ of $\Eventually^{\abs}p$  whenever  $\Eventually^{\abs}p$ is asserted at a position of an infinite \MAP.

We now provide the formal definition of $\Au_{y^{\abs}_p}$. For this, we need additional notation. An \emph{obligation set} $O$ (for the fixed predictor event-clock $y^{\abs}_p$) is a set consisting of lower-bound
obligations $\succ $$\ell$ and upper-bound obligations  ($f$,$\prec$$u$), where $f\in \{\live,\first\}$, such that
$y_p^{\abs} \succ \ell$ and $y_p^{\abs} \prec u$ are constraints of $\Au$, and $(f,\prec$$u), (f',\prec$$u)\in O$ implies $f=f'$.
For an obligation set $O$, $\live(O)$ is the obligation set obtained by $O$ by removing all the obligations which are \emph{not} of the form $(\live, \prec$$u)$ (i.e., $\live(O)$ consists of the live upper-bound obligations of $O$). A \emph{check set} $K$ is a subset of $\{\call,\ret,\intA,\Eventually^{\abs} p,p_{\infty}\}$ such that
$K\cap \{\call,\ret,\intA\}$ is a singleton. For an input symbol $a\in \Sigma_\Prop$ and an obligation set $O$, we denote by $\con(O,a)$ the constraint over the new set $C_\new$ of normal clocks defined as:
$\con(O,a)=\true$ if either $O=\emptyset$ or $p\notin a$; otherwise, $\con(O,a)$ is obtained from $O$ by adding for each obligation $\succ \ell$ (resp., $(f,\prec$$ u)$), the conjunct $z_{\succ \ell}\succ \ell$
(resp., $z_{\prec u}\prec u$).
The nested \VPTA\ $\Au_{y^{\abs}_p}$ is given by
%
\[
\Au_{y^{\abs}_p}= \tpl{\Sigma_\Prop, Q',Q'_{0},C\setminus\{y^{\abs_p}\}\cup C_n \cup C_{\new},Q'\cup\{\bad,\top\},\Delta',\mathcal{F}'}
 \]
%
 where the set $Q'$ of states consists of triples of the form $(q,O,K)$ such that $q$ is a state of $\Au$,
$O$ is an obligation set, and $K$ is a check set. The set $Q'_0$ of initial states consists of states of the form $(q_0,\emptyset,K)$ such that $q_0\in Q_0$ (initially there are no obligations).


We now define the transition function $\Delta'$. For this, we first define a predicate $\Abs$ over tuples $\tpl{(O,K),a, y_p^{\abs}\in I,\Res,(O',K')}$
where $(O,K),(O',K)$ are pairs of obligation sets and check sets, $a\in\Sigma_\Prop$, $y_p^{\abs}\in I$ is a constraint of $\Au$, and $\Res\subseteq C_\new$. Intuitively, $O$ (resp., $K$) represents the obligation set (resp., check set)  at the current position $i$ of the input, $a$ is the input symbol associated with position $i$, $y_p^{\abs}\in I$ is the prediction about $y_p^{\abs}$ done by $\Au$ at position $i$,
$\Res$ is the set of new normal clocks reset by $\Au_{y^{\abs}_p}$ on reading $a$,
 and
$O'$ (resp., $K'$) represents the obligation set (resp., check set) at the position $j$ following $i$ along the \MAP\ visiting  $i$ (if $i$ is a call, then $j$ is the matching-return of $i$). Formally,
$\Abs((O,K),a, y_p^{\abs}\in I,\Res,(O',K'))$ iff the following holds:
  \begin{enumerate}
  \item ($p_{\infty}\in K$ iff $p_{\infty}\in K'$), $K\cap \{\call,\ret,\intA\}\subseteq a$.
  \item $\Eventually^{\abs} p\in K$ iff ($p\in a$ or $\Eventually^{\abs} p\in K'$), and ($\Eventually^{\abs} p \in K'$ iff $I\neq\{\NULL\}$).
  \item If $I=\{\NULL\}$, then   $O'=\live(O)$, $\Res =\emptyset$, and $p\notin a$ implies $O=\live(O)$. Otherwise, let
   $y_p^{\abs}\in I \equiv y_p^{\abs}\succ \ell \wedge y_p^{\abs} \prec u$.  Let $O''$ be $O$ if $p\notin a$, and $O''=\live(O)$ otherwise. Then, $O' = O'' \cup \{ \succ$$ \ell\} \cup \{ (f, \prec$$ u)\}$, where $f= \live$ if $(\live, \prec$$ u)\in O''$, and $f=\first$ otherwise. Moreover, $\Res\subseteq \{z_{\succ \ell},z_{\prec u}\}$, $z_{\succ \ell}\in\Res$, and $z_{\prec u}\in \Res$ iff either
    $\prec$$ u$ does not appear in $O$, or $p\in a$ and $(\first,\prec$$ u)\in O$.
   \end{enumerate}
%
Condition~1 requires that the Boolean value of proposition $p_{\infty}$ is invariant along the positions of a \MAP, and
the current check set is consistent with the type (call, return, or internal symbol) of the current input symbol.
Condition~2 provides the abstract-local propagation rules of formula $\Eventually^{\abs} p$.
Finally, Condition~3 provides the rules for how the obligations are updated on moving to the abstract next position along the current \MAP\ and what new clocks have to be reset on reading the current input symbol
$a$. Note that if $I=\{\NULL\}$ and $p\notin a$, then the current obligation set must contain only live upper-bound obligations. If instead
$y_p^{\abs}\in I$ is equivalent to  $y_p^{\abs}\succ \ell \wedge y_p^{\abs} \prec u$, then   the clock $z_{\succ \ell}$ is  reset, while the clock
$z_{\prec u}$ is reset iff either there is no obligation $(f,\prec$$u)$ in $O$, or $p\in a$  and the obligation $(f,\prec$$u)$ is fresh, i.e., $f=\first$.

  The transition function $\Delta'$ of $\Au_{y^{\abs}_p}$  is then defined as follows. Recall that we can assume that each clock constraint of $\Au$ is of the form
$\theta \wedge y_p^{\abs}\in I$, where $\theta$ does not contain occurrences of $y_p^{\abs}$.

\paragraph{Push transitions:} for each push transition $q\, \der{a,\theta \wedge y_p^{\abs}\in I, \Res,\push(\gamma)}\,q'$ of $\Au$, we have the push  transitions
$(q,O,K) \, \der{a,\theta\wedge \con(O,a), \Res\cup\Res',\push(\gamma')}\,(q',O',K')$ such that
%
\begin{enumerate}
\item Case $\gamma'\neq \bad $. Then,   $\gamma'=(\gamma,O_{\ret},K_{\ret})$  and
  \begin{compactitem}
 \item $\Abs((O,K),a,y_p^{\abs}\in I,\Res',(O_{\ret},K_{\ret}))$. Moreover, if $\ret\in K'$ then  $K_{\ret} =K'$ and $O'=\emptyset$; otherwise, $p_{\infty}\notin K'$  and $O'$ consists of the live  obligations
  $(\live,\prec $$u)$ such that  $(f,\prec $$u)\in O_{\ret}$ for some $f\in \{\live,\first\}$.
 \end{compactitem}
   \item Case $\gamma'= \bad$: $\call\in K$, $I=\{\NULL\}$, ($\Eventually^{\abs} p\in K$ iff $p\in a$), $p_{\infty}\in K$, $p_{\infty}\in K'$, $\ret\notin K'$, $O'=\emptyset$, $\Res'=\emptyset$, and $p\notin a$  implies $O=\emptyset$.
\end{enumerate}
%
Note that if $p\in a$, the obligations in the current state are checked by the constraint on $C_\new$ given by $\con(O,a)$ (recall that if $p\notin a$, then $\con(O,a)=\true$). The push transitions of point~1 consider the case  where $\Au_{y^{\abs}_p}$ guesses that the current call position $i_c$ has a matching return $i_r$. In this case, the set of obligations and the check state for the next abstract position $i_r$ along the current \MAP\ are pushed on the stack in order to be recovered at the matching-return $i_r$. Moreover, if $\Au_{y^{\abs}_p}$ guesses that the next position $i_c+1$ is not $i_r$ (i.e., $\ret\notin K'$), then all the upper-bound obligations in $O_{\ret}$ are propagated as  live obligations at the next position $i_c+1$ (note that the \MAP\ visiting $i_c+1$ starts at $i_c+1$, terminates at $i_r-1$, and does not satisfy proposition $p_{\infty}$).
The push transitions of point~2 consider instead the case  where $\Au_{y^{\abs}_p}$ guesses that the current call position $i_c$ has no matching return $i_r$, i.e., $i_c$ is the last position of the current \MAP. In this case, $\Au_{y^{\abs}_p}$ pushes the symbol $\bad$ on the stack and the transition relation is consistently updated.

\paragraph{Internal transitions:} for each internal transition $q\, \der{a,\theta \wedge y_p^{\abs}\in I, \Res}\,q'$ of $\Au$, we add   the internal transitions
$(q,O,K) \, \der{a,\theta\wedge \con(O,a), \Res\cup\Res'}\,(q',O',K')$, where
%
\begin{enumerate}
  \item Case $\ret\in K'$: $\intA\in K$,  $I=\{\NULL\}$, $\Res' = \emptyset$, $O'=\emptyset$, ($\Eventually^{\abs}p\in K $ iff $p\in a$), and $p\notin a$ implies $O=\live(O)$.
  \item Case $\ret\notin  K'$:  $\Abs((O,K),a, y_p^{\abs}\in I,\Res',(O',K'))$.
\end{enumerate}
In the first case, $\Au_{y^{\abs}_p}$ guesses that
the current internal position $i$ is the last one of the current \MAP ($\ret\in K'$), while in the second case  the current \MAP\ visits the next non-return position $i+1$.
Note that if $p\in a$, the obligations in the current state are checked by the constraint $\con(O,a)$.
%
\paragraph{Pop transitions:} for each pop transition $q\, \der{a,\theta \wedge y_p^{\abs}\in I, \Res,\pop(\gamma)}\,q'\in \Delta_r$, we have the pop  transitions
$(q,\emptyset,K) \, \der{a,\theta\wedge \theta', \Res\cup\Res',\pop(\gamma')}\,(q',O',K')$, where
%
\begin{enumerate}
  \item Case $\gamma\neq \top$: $\ret\in K$, $\gamma'=(\gamma,(O_{\ret},K))$, and  $\theta'= \con(O_{\ret},a)$.
  If $\ret\notin K'$, then  $\Abs((O_{\ret},K),a, y_p^{\abs}\in I,\Res',(O',K'))$; otherwise, $I = \{\NULL\}$, $\Res'=\emptyset$, $O'=\emptyset$,
  ($\Eventually^{\abs} p\in K$ iff $p\in a$), and $p\notin a$ implies $O_{\ret}= \live(O_{\ret})$.
\item Case $\gamma = \top$: $\ret\in K$,   $\gamma'=\top$, $\theta'=\true$, $p_{\infty}\in K$, and $p_{\infty}\in K'$.
If $\ret\notin K'$, then  $\Abs((\emptyset,K),a, y_p^{\abs}\in I,\Res',(O',K'))$; otherwise, $I = \{\NULL\}$, $\Res'=\emptyset$, $O'=\emptyset$, and
  ($\Eventually^{\abs}p\in K$ iff $p\in a$).
\end{enumerate}
%
If $\gamma\neq \top$, then the current return position has a matched-call. Thus, $\Au_{y^{\abs}_p}$ pops from the stack the obligations
$O_{\ret}$ at the current position and if $p\in a$, check that they are satisfied by the constraint $\con(O_{\ret},a)$. If $\gamma = \top$, then the current position is also the initial position
of the associated \MAP.

Finally, the generalized B\"{u}chi condition $\mathcal{F}'$ of $\Au_{y^{\abs}_p}$ is defined as follows. For each B\"{u}chi component $F$ of $\Au$,
 $\Au_{y^{\abs}_p}$  has the B\"{u}chi component consisting of the states $(q,O,K)$ such that $q\in F$. Moreover,
  $\Au_{y^{\abs}_p}$ has an additional component consisting of the states $(q,O,K)$ such that $p_{\infty}\in K$, and either $\Eventually^{\abs}p\notin K$ or $p\in K$.
 Such a component  ensures that  the guesses about the matched calls are correct ($p_{\infty}$ occurs infinitely often), and that  the liveness requirement
$p$ of $\Eventually^{\abs}p$ is fulfilled whenever  $\Eventually^{\abs}p$ is asserted at a position of an infinite \MAP. Note that in an infinite word over $\Sigma_\Prop$, there are at most one
infinite  \MAP\ $\nu$ and $\nu$ visits only positions where $p_{\infty}$ holds; moreover,   each position $i$ greatest than the initial position
$i_0$ of $\nu$ is either a $\nu$-position, or a position where $p_{\infty}$ does not hold.




